Physics Opportunities at a Beam Dump Facility at PIP-II at Fermilab and Beyond

The Fermilab Proton-Improvement-Plan-II (PIP-II) is being implemented in order to support the precision neutrino oscillation measurements at the Deep Underground Neutrino Experiment, the U.S. flagship neutrino experiment. The PIP-II LINAC is presently under construction and is expected to provide 800~MeV protons with 2~mA current. This white paper summarizes the outcome of the first workshop on May 10 through 13, 2023, to exploit this capability for new physics opportunities in the kinematic regime that are unavailable to other facilities, in particular a potential beam dump facility implemented at the end of the LINAC. Various new physics opportunities have been discussed in a wide range of kinematic regime, from eV scale to keV and MeV. We also emphasize that the timely establishment of the beam dump facility at Fermilab is essential to exploit these new physics opportunities.

==> Contributions/neutrinos.tex <==
\subsection{Neutrinos as Signal and as Background - {\bf Vishvas Pandey}}

Protons with energies $>$ 300 MeV produce large numbers of pions, these pions can lose energy in dense material, stop and decay after coming to rest.  Clean stopped-pion neutrinos can be produced with proton energies of the order of 1 GeV or less~\cite{Alonso:2010fs}~(that limits the decay-in-flight component), and with a dense target to allow the pions to stop and decay at rest. The dominant neutrino production from stopped pions is from the weak-interaction two-body \textit{prompt} decay $ \pi^{+} \rightarrow \mu^+ + \nu_\mu$  ($\tau \sim$ 26 ns) followed by a three-body \textit{delayed} decay of muons $\mu^{+} \rightarrow e^+ + \nu_e + \bar{\nu}_\mu$ ($\tau \sim$ 2.2 $\mu$s) producing a well know spectrum shape. The prompt $\nu_\mu$ is monoenergetic (29.8 MeV) while $\nu_e$s and $\bar{\nu}_\mu$s energies spread out upto $m_\mu/2$. The stopped pion decay spectrum is relatively well known,  radiative corrections to pions and muons decaying at rest account for a tiny fraction of additional uncertainty~\cite{Tomalak:2021lif}. \\

These tens of MeV neutrinos can scatter off the target nucleus in the detector either via (i) neutral current coherent elastic neutrino-nucleus scattering (CEvNS) producing keV scale energy nuclear recoil signature, or (ii) charged current (only $\nu_e$s) or neutral current (all favors) inelastic scattering producing MeV scale energy signatures. These neutrinos can be treated as a signal for various SM and BSM studies, and they form the background to various BSM physics signals. The pulsed time structure of these neutrinos gives a strong handle on suppressing the background.

\subsubsection{Elastic Scattering and keV Scale Physics}

In the CEvNS case, the neutrino scatters off an entire nucleus, exchanging a $Z^0$ boson transferring some of its momenta to the nucleus as a whole, the scattered nucleus remains in its ground state.  For few tens of MeV energy neutrinos and scattering off medium-sized nuclei, a dominant fraction of interactions are expected to be of coherent type. The differential cross section of the process is written as:
%
\begin{equation}\label{Eq:cevns_xs}
\frac{\mathrm{d}\sigma}{ \mathrm{d}T} = \frac{G^{2}_{F}}{\pi} M_{A} \left(1-\frac{T}{E_{\nu}}-\frac{M_A T}{2 E^2_\nu}\right)~\frac{Q^2_{W}}{4}~F_{W}^2(Q^2), 
\end{equation}
%
where $G_F$ is the Fermi coupling constant, and $Q_W$ is the weak nuclear charge given as $Q^{2}_{W} = [g_p^V Z+g_n^V N]^2 = [(1-4\sin^2\theta_\text{W}) Z-N]^2$. N (Z) are neutron (proton) numbers, $\theta_W$ is the weak mixing angle, $E_\nu$ is the neutrino energy, $T$ is the nuclear recoil energy, and $M_A$ is the nuclear target mass. $F_{W}^2(Q^2)$ is the weak form factor of the nucleus. The weak-interaction charge of the proton is small compared to that of the neutron, so the CEvNS rate primarily depends upon $N^2$, the square of the number of neutrons. \\

The uncertainty on the CEvNS cross section is dominated by the weak form factor of the nucleus and is estimated to be a few percent level~\cite{VanDessel:2020epd}, the radiative corrections form a tiny fraction of the total uncertainty~\cite{Tomalak:2020zfh}. Since the uncertainties on SM predicted CEvNS cross section is relatively small, CEvNS cross section measurements allow testing of SM weak physics (e.g. weak nuclear form factor of a nucleus and weak mixing angle) or probing many new physics signals (e.g. non-standard interactions, sterile neutrinos, light dark matter) where CEvNS form the primary irreducible background. Any deviation from the SM predicted event rate either with a change in the total event rate or with a change in the shape of the recoil spectrum, could indicate new contributions to the interaction cross-section. The experimental signature of CEvNS is low-energy nuclear recoils $T$ of $\mathcal{O}$(keV). The pulsed time structure of these neutrinos gives a strong handle on suppressing the background for BSM physics signals. The detectors with keV energy threshold are discussed in Sec.~[]. 

\subsubsection{Inelastic Scattering and MeV Scale Physics}

In the inelastic NC or CC scattering, where a single $W^+$ (CC) or $Z^0$ (NC) boson is exchanged between neutrino and target nucleus, the neutrino excites the target nucleus to a low-lying nuclear state, followed by nuclear de-excitation products such as gamma rays or ejected nucleon. The interaction cross sections for these processes do not have the $N^2$ enhancement therefore they are typically  an order of magnitude smaller than that of CEvNS process. The observable final-state particles of these inelastic scattering have typical energies of the same order as the incident neutrino energies, $\mathcal{O}$(MeV). Inelastic neutrino-nucleus cross-sections in these tens of MeV regime are quite poorly understood. Theoretical understanding of these processes is also relatively poor, due to the strong dependence of the interaction rates on the specific initial- and final-state nuclear wavefunctions, and experimental measurements are sparse~\cite{VanDessel:2020epd, Pandey:2014tza, Pandey:2016jju}. The neutrinos from the galactic core-collapse supernova carry similar energies as the well-understood stopped-pion neutrinos, therefore measuring inelastic neutrino interaction off nuclei (in particular off argon) can provide a unique opportunity to enable future neutrino experiments' (e.g. DUNE) capability to detect supernova neutrinos~\cite{DUNE:2023rtr}, please see Sec.~[LArTPC…]. \\

In addition to probing standard model nuclear structure physics and enabling supernova detection capabilities, inelastic neutrino-nucleus scattering also forms the irreducible background to some BSM signals including ALP and inelastic DM-nucleus scattering that produce similar MeV scale signature. Alternate to widely explored elastic scattering keV scale signals of e.g. dark photon models, the inelastic scattering of the same DM candidates has a smaller cross section but the MeV scale gamma rays signature can have higher signal-to-background ratios~\cite{Dutta:2023fij, Dutta:2022tav}. The decay of nuclei excited by the inelastic scattering of DM is an unexploited channel that has a significantly lower background compared to similar searches using the elastic scattering channel. These models can be explored at decay at rest facilities using detectors with MeV scale signal sensitivity. The detectors with MeV energy threshold are discussed in Sec.~[]. 
